Decentralized Collaborative Inertial Tracking

Although people spend most of their time indoors, outdoor tracking systems, such as the Global Positioning System (GPS), are predominantly used for location-based services. These systems are accurate outdoors, easy to use, and operate autonomously on each mobile device. In contrast, Indoor Tracking Systems~(ITS) lack standardization and are often difficult to operate because they require costly infrastructure. In this paper, we propose an indoor tracking algorithm that uses collected data from inertial sensors embedded in most mobile devices. In this setting, mobile devices autonomously estimate their location, hence removing the burden of deploying and maintaining complex and scattered hardware infrastructure. In addition, these devices collaborate by anonymously exchanging data with other nearby devices, using wireless communication, such as Bluetooth, to correct errors in their location estimates. Our collaborative algorithm relies on low-complexity geometry operations and can be deployed on any recent mobile device with commercial-grade sensors. We evaluate our solution on real-life data collected by different devices. Experimentation with 16 simultaneously moving and collaborating devices shows an average accuracy improvement of 44% compared to the standalone Pedestrian Dead Reckoning algorithm.

==> sections/method.tex <==
\todo{These two sections should be merged}
\section{Method}

We will leverage the extended advertising extension offered by Bluetooth 5 to exchange packets. 
With the new Bluetooth 5 specification, packets can be chained together to form an even larger payload of a maximum of 1650 bytes.

We need to tackle a connection deprivation attack by setting a timeout of X seconds.

\section{Methodology}
Our approach consists in exploiting \gls{pdr} solutions that achieves a given accuracy by considering the impact of drift. We observe that the error still accumulate as time goes. 

To fix the drifting problem in existing INS-based ITS, we integrate a BLE-sensor available on new devices. BLE allows us to exchange small data within a short range while preserving a power consumption.
